A Simple and General Operational Framework to Deploy Optimal Routes with Source Routing

Source Routing, currently facilitated by Segment Routing (SR), enables precise control of forwarding paths by specifying detours (or segments) to deviate IP packets along routes with advanced properties beyond typical shortest IGP paths. Computing the desired optimal segment lists, known as encoding, leads to interesting challenges as the number of detours is tightly constrained for hardware performance. Existing solutions either lack generality, correctness, optimality, or practical computing efficiency-in particular for sparse realistic networks. In this paper, we address all such challenges with GOFOR-SR. Our framework extends usual path computation algorithms to inherently look at optimal and feasible segment lists, streamlining the deployment of TE-compliant paths. By integrating encoding within the path computation itself and modifying the distance comparison method, GOFOR allows algorithms with various optimization objectives to efficiently compute optimal segment lists. Despite the loss of substructure optimality induced by SR, GOFOR proves particularly efficient, inducing only a linear overhead at worst. It also offers different strategies and path diversity options for intricate TE-aware loadbalancing. We formally prove the correctness and optimality of GOFOR, implement our framework for various practical usecases, and demonstrate its performance and benefits on both real and challenging topologies.

==> ethics.tex <==
%\section*{Ethical Issues}

\vspace*{0.2cm}
\emph{Note: This work raises no ethical issues.}


==> exemple-FRR.tex <==
\begin{tikzpicture}[-,>=stealth',shorten >=1pt,node distance=3cm,
            thick,main node/.style={circle,inner sep=3pt,draw,font=\sffamily},
            edgelabel/.style={fill=white,inner sep=2pt, anchor=center, pos=0.5,font=\sffamily},
            yscale=0.8, xscale=0.8
            %,every node/.append style={transform shape}
            ]
    
        \node[main node, fill={rgb:black,1;white,5}] (S) at (0,0) {S};
        \node[main node, fill={rgb:black,1;white,5}] (D) at (6,0) {D};
        \node[main node] (2) at ($(S)!0.5!(D)$) {2};

        \node[main node] (5) at (7,1.5) {5};
        \node[main node] (4) at (3,3.7) {4};
        \node[main node] (1) at (1.5,1.5) {1};
        \node[main node] (3) at (4.5,1.5) {3};
        \node[main node] (6) at (0.7,2.7) {6};
        \node[main node] (7) at (5.3,2.7) {7};

        \path 
        (S) edge node[cross, anchor=center] {} (2)
        (S) [->, bend left=20] edge[draw=cyan] node[edgelabel] {10} (1)
        (S) [-,bend left=20] edge[draw=cyan] node[edgelabel] {20} (6)
    
        (1) [->, bend left=20] edge (S)
        (1) [->, bend left=20] edge[draw=cyan] node[edgelabel] {10} (3)
    
        (2) [-,bend left=0] edge node {} (D)
    
        (3) [->,bend left=20] edge  (1)
        (3) [-,bend left=20] edge[draw=cyan] node[edgelabel] {10} (D)
    
        (4) [-,bend left=10] edge[draw=cyan] (7)
    
        (5) [-,bend left=10] edge[draw=cyan] node[edgelabel] {4} (D)
    
        (6) [-,bend left=10] edge[draw=cyan] (4)
    
        (7) [-] edge[draw=cyan] node[edgelabel] {4} (5)
        (7) [-,bend left=20] edge[draw=cyan] node[edgelabel] {8} (D)
    
        (D) [->,bend left=20] edge[draw=black] (3);
    
        \end{tikzpicture}

==> lca.tex <==


\begin{figure}
  \centering
  \begin{tabular}{cl} \toprule
      \textsc{notation} & \textsc{definition}\\
      \toprule
      $(u,v)$ & An edge in $E$ between node $u$ and $v$\\
      $w(u,v)$ & The weight vector of edge $(u,v)$\\
      $w_i(u,v)$ & The $i^{th}$ component of $w(u,v)$\\
      \midrule
      $p(s,t)$ & A path between node $s$ and $t$,\\ 
      &defined as a list of edges\\
      $p_{[x_i, x_j]}$ & A subpath of $p$, defined as \\
      & a list of edges belonging to $p$.\\
      $d(p)$ & The distance vector of path $p$.\\
      $d_i(p)$ & The $i^{th}$ component of $d(p)$, $i \leq m$.\\
      $Dag_{[u]}$ & Set of edges forming the shortest \\
      & IGP path DAG rooted at $u$\\
      $Dag_{[u,v]}$ & Edges of the paths from $u$ to $v$\\
      & within $Dag_{[u]}$\\
      \midrule
      $P_i^*(s,t)$ & All shortest path between node $s$ and $t$\\
      & when considering the $i^{th}$ criterion.\\
      $d_i^*(s,t)$ & The best distance between node $s$ and $t$\\
      & when considering the $i^{th}$ criterion.\\
      $d_i^{max}(P(s,t))$ & The maximum distance among all paths \\
      & $p \in P$ considering the $i^{th}$ criterion\\
      \midrule
      $S$ & A segment list\\
      $S_i = (t, s_i, s_{i+1})$ & A segment encoding a path between \\
      & $u$ and $v$ with $t = {Adj, Node}$\\
      $S_{\left[i,j\right]}$ & Sublist of $S$ consisting in ${S_i, \dots ,S_j}$\\
      $d^{SR}(t, s_i, s_{i+1})$ & The best distances guaranteed by\\
      & a segment $(t, s_i, s_{i+1})$\\
      $d^{SR}(S)$ & Distances of a segment list, defined as\\
      & the sum of the distances of \\
      &each segment. \\
      \bottomrule
      
  \end{tabular}
  \caption{Notations}
\end{figure}\label{tab:notationslca}




We first describe the problem, then we present the algorithm and finally we show how to use it to compute Delay-Constrained-Least-Cost paths.



The common goal of path encoding schemes is to find, given an input path, a segment list encoding said path with the minimum number of segments. However, there exist several paradigms one may follow to compute segment lists.


Most path encoding schemes aim to encode a single, specific path (as described in Section~\ref{ssec:path-encoding}). In other words, the (usually minimal) segment list computed \emph{solely} encodes the input path. We refer to this as \emph{strict encoding}. When considering a single metric, strict encoding makes sense. Indeed, in this case, SR is usually used for goals such as path monitoring, failure resiliency, or function chaining. It is thus important that traffic follows exactly the desired path.

In our case, we argue that while the input path should be considered, its \emph{distance} is what matters most. Load-balancing should thus be leveraged, as long as the delay constraint is respected. In this case, two main paradigms can be followed. The first one consists in providing a distance as input and returning a segment list encoding any path(s) with said distance (at most). We refer to this approach as \emph{weak encoding}. The second approach consists in returning a segment list that \emph{does} encode a path given as input, but may also encode other paths sharing the same or better distances. We refer to this approach as \emph{strong encoding}.\\



% \begin{figure*}
%     \centering
%     \includegraphics[scale=0.6]{./figures/encodings-3.pdf}
%     \caption{Figure illustrating the different type of encodings}\label{fig:encodings}
% \end{figure*}


The different types of encodings are illustrated in Fig.~\ref{fig:encodings}. Given the path to encode $p$, the segment lists $S$ resulting from each type of encoding are shown. The paths encoded by $S$ are shown in their respective color on the left side of the Figure.

We consider the path $p = (s,a),(a,b),(b,d)$. When relying on strict encoding, three segments are necessary to circumvent the effect of ECMP. Several segment lists weakly encode $p$, \ie encode path with distance $d = (10,10)$. Within these lists, the minimal one is composed of a single segment, encoding a direct edge between $s$ and $d$. Note that the original path $p$ is not contained within this segment list. Finally, the segment list that strongly encodes $p$ does indeed encode $p$, as well as another path of equal distance. 

While weak encoding may seem like the most natural option, it has several caveats. First, from a technical standpoint, its outcome is far less predictable, as it solely depends on distance with no paths acting as general anchor points. Second, weakly encoding a given distance $d(p = (s,t))$ may induce a high computational complexity. Intuitively, the lack of anchor points around which building the segment list requires finding all paths with said distance to find the associated minimal segment lists. In addition, note that relying on strong encoding does not necessarily prevent finding minimal encoding segment lists, as long as the proper path is considered. For example, considering Fig.~\ref{fig:encodings}, the encoding $S = (Adj, s_2, d)$ may also be found by strongly encoding the non-dominated path $p = (s_2, d)$. We leverage this when designing our conversion algorithm, in order to benefit from the more efficient strong encoding paradigm, while still ensuring that the minimal segment list is retrieved.\\


We thus design \lca as a conversion algorithm following the \emph{strong encoding} paradigm. We first devise an offline conversion algorithm returning the minimal strongly encoding segment lists for a given path. We then adapt this algorithm for it to be usable online, \ie to encode paths \emph{while} exploring the graph. We show that the peculiarities of the segment metric require particular care when maintaining and extending the distances. In particular, we show that some dominated distances must now be extended, as their number of segments may evolve differently despite being extended by the same edge. From there, we formally define how distances should be maintained (in particular when following the strong encoding paradigm), in order to ensure retrieving the actual 3D Pareto front, with the minimal encoding segment list of each non-dominated distance.\\



As the descriptions of \lca  and strong encoding rely heavily on the notations introduced previously,  we start by introducing (or reminding of) the following notations. We consider a network $G = (V,E)$. Let $p = ((x_0, x_1),(x_1, x_2), \dots,(x_{l-1}, x_l))$ be a path within $G$, with $x_i \in V$. Let $p_{[x_i, x_j]} = ((x_i, x_{i+1}),\dots, (x_{j-1}, x_j))$. We here consider the distance $d(p)$ as $d(p) = (d_1(p), d_2(p))$, as $d_0$ is unknown. 



We denote $P^*_2(u,v)$ all the shortest paths between $u$ and $v$ in $G$ with respect to the $M_2$ metric (\ie all ECMP paths between $u$ and $v$). The edges of the paths $P^*_2(u,v)$ form a subgraph of the shortest path DAG rooted at $u$ (considering $M_2$). We denote $\mathit{Dag}_{[u,v]}$ this set of edges.


A segment is characterized by a tuple $(t,u,v)$, which encodes all ECMP paths from $u$ to $v$ when $t = Node$, or a specific link when $t = Adj$. We denote $d^{SR}(t, u, v)$ the best distances guaranteed when following the paths encoded by the segment $(t,u,v)$. When $t = Node$, we have $d^{SR}(t, u, v) = (d_1^{max}(P^*_2(u,v)),d_2^*(u,v))$. When $t = Adj$, we have $d^{SR}(t, u, v) = w(u,v)$. Notice that the distance $d^{SR}$ of a segment is thus exactly equal to the weight of the edge associated to this segment in the SR Graph.

Finally, we denote a list of segments $S = (S_i)_{0 \leq i \leq l-1}$. 
A segment $S_i \in S$ is thus defined as a tuple $(t_i, s_i, s_{i+1})$, with $s_i \in V$ and $t_i \in \{\mathit{Adj}, \mathit{Node}\}$.  We defined the distance of a segment list $d^{SR}(S) = \sum_{n = 0}^{l-1} d^{SR}(S_i)$.





We now define formally the \emph{strong encoding} of a path $p$.

\begin{Definition}[Strong Encoding]~\label{def:encoding}
  Let $p = ((x_0,x_1),\dots,(x_{l-1},x_l))$ be a path. Let $S = (S_i)_{0 \leq i \leq l-1}$ be a segment list. $S$ \emph{strongly encodes} the path $p$ if both conditions are verified:
  \begin{itemize}
    \itemsep0em
    \item $\forall i$, $\exists j$ such that $s_i = x_j$
    \item $\forall i$, either 
    \begin{enumerate}[label={(\roman*)}]
      \itemsep0em
      \item $p_{[s_i, s_{i+1}]} \in P_2^*(s_i, s_{i+1})$ and $d(p_{[s_i, s_{i+1}]})$ is dominated by $d^{SR}(S_i)$, or
      \item $t_i = \mathit{Adj}  \wedge (s_i, s_{i+1}) \in p$.
    \end{enumerate}
  \end{itemize} 
\end{Definition}

Less formally, Def.~\ref{def:encoding} ensures that each segment within a segment list $S$ either (i) does indeed encode a subpath of $p$, and that the paths encoded by the segment have equal or better distances than said subpath or (ii) encodes a specific link within $p$. 

\begin{Remark}\label{rem:strenc}
When considering condition (i) of Def.~\ref{def:encoding}, $p_{[s_i, s_{i+1}]}$ and $d(S_{[i, i+1]})$ necessarily share the same cost $d_1$ (the cost of the ECMP paths from $s_i$ to $s_{i+1}$, $d^*_2(s_i, s_{i+1})$). 

Furthermore, by definition, the delay of $S_{[i, i+1]}$ is equal to the \emph{maximum} delay among all ECMP paths within $P^*_2(s_i, s_{i+1})$. 
Thus, stating that  $d(p_{[s_i, s_{i+1}]})$ is dominated by $d(S_{[i, i+1]})$, is equivalent to stating that $d_1(p_{[s_i, s_{i+1}]}) = d_1(S_{[i, i+1]}) = d_1^{max}(P_2^*(s_i, s_{i+1}))$. 

Consequently, (i) can be alternatively expressed as : $$d(p_{[s_i, s_{i+1}]}) = d(S_{[i, i+1]}).$$
\end{Remark}




We then define the \emph{delay-cost path encoding problem}, which we aim to solve with our encoding scheme.

\begin{Definition}[Delay-cost path encoding problem]
Given a path $p$, the delay-cost path encoding problem consists in finding a segment list $S$ that strongly encodes $p$ with the minimal number of segments.
\end{Definition}


Before describing how we solve the Delay-cost path encoding problem in an online fashion (\ie while exploring the graph), we first describe how to solve this problem when the complete path is already known and provided as input.\\


We solve the delay-cost path encoding problem through a greedy algorithm. In short, this algorithm repeatedly finds, for a given path $p$, the longest prefix of $p$ encodable by a single segment. This algorithm is presented in Alg.~\ref{algo:encode}.


\SetKwRepeat{Do}{do}{while}
\begin{algorithm}
  \footnotesize
  \caption{ \footnotesize \textsc{encode}($p$)}\label{algo:encode}
  $s := x_0$\\
  $S := [~]$\\
  \Do{$s \neq x_l$}{
    $S_i = (t, s, v)$ = 1SegLongestPrefix($p_{[s, x_l]}$)\\
    $S$.push($S_i$)\\
    $s := v$\\
  }
  \Return $S$
  
\end{algorithm}


Considering a path to encode $p$ and a source $s$ (the first node of the path), Alg.~\ref{algo:encode} starts by finding the longest prefix of $p$ encodable in a single segment. Suppose that $S_i$ encodes such a prefix $p_{[s, v]}$. The algorithm then adds the segment to the segment list $S$ and repeats the procedure, considering the remainder of the path $p_{[v, x_l]}$ and $v$ as the new source. This is repeated until the node considered as source is equal to the last node in $p$, \ie $x_l$.\\




\begin{algorithm}
  \footnotesize
  \caption{\footnotesize \textsc{1SegLongestPrefix}($p = (x_0, x_1), \dots (x_{l-1}, x_l)$)}\label{algo:1SLP}
  %\If{$SR(x_0, x_1) \lneq d(p[x_0,x_1]$)}{ \label{test1}
%   \If{$(x_0,x_1) \notin \mathit{Dag}_{[x_0,x_1]}$ \textbf{or} $w_1(x_0,x_1) \leq d_1^{max}(P^*_2(x_0, x_1))$}{\label{test1}
  \If{$(x_0,x_1) \notin \mathit{Dag}_{[x_0,x_1]}$ \textbf{or} $w_1(x_0,x_1) \leq d_1^{SR}(Node,x_0, x_1)$}{\label{test1}
      \Return $(\mathit{Adj}, x_0, x_1)$\label{algo:enc:return1}\\
  }


  \For{$i = 2\dots l$}{
    \If{$(x_{i-1}, x_i) \notin \mathit{Dag}_{[x_0, x_i]}$ \textbf{or} $d_1(p_{[x_0, x_i]}) < d_1^{SR}(Node, x_0, x_i)$}{\label{test2}
      \Return $(\mathit{Node}, x_0, x_{i-1})$\label{algo:enc:return2}\\
    }
  }
  \Return $(\mathit{Node}, x_0, x_l)$\label{algo:enc:return3}\\

\end{algorithm}






To find the longest prefix encodable in one segment (and the associated segment), Alg~\ref{algo:encode} relies on another algorithm, \textsc{1SegLongestPrefix}, described in Alg.~\ref{algo:1SLP}. Intuitively, Alg.~\ref{algo:1SLP} tries to encode as many edges of $p$ as possible in a single segment. Once the algorithm detects that a new segment would be required to properly encode an additional edge (\eg because it deviates from the ECMP paths), the algorithm returns.




More precisely, \textsc{1SegLongestPrefix} starts by checking whether the first edge of $p$ requires an adjacency segment (Line~\ref{test1}). Recall that a node segment may only encode ECMP paths, \ie paths within $P^*_2$. Consequently, a node segment (interpreted by $x_0$) may not encode an edge $(x_0,x_1)$ which does not lies within $\mathit{Dag}_{[x_0, x_1]}$. In this case, the edge $(x_0,x_1)$ must be encoded by an adjacency segment~\footnote{If several adjacency segments exist between $x_0$ and $x_1$, the one that matches the weight of the considered edge should be used.}. Note that since an adjacency segment only encodes a single link, encoding additional edges will necessarily require new segments. Hence, the algorithm returns immediately. 


Otherwise, the algorithms checks, for each $i = 2\dots l$, whether the subpath $p_{[x_0, x_i]}$ \emph{remains} encodable in a single node segment when considering an additional edge $(x_{i-1}, x_i)$. To remain encodable in a single node segment, the subpath must respect two conditions.

First, it must remain an ECMP path. This can be checked by verifying whether the new edge $(x_{i-1}, x_i)$ remains within the shortest path DAG rooted at $\mathit{Dag}_{x_0}$, \ie if the edge belongs to $\mathit{Dag}_{x_0, x_i}$. Otherwise, the subpath induced by the added edge deviates from the shortest paths rooted at $x_0$ and thus cannot be encoded through a node segment interpreted by $x_0$. Second, if it is an ECMP path from $x_0$ to $x_i$, it must not possess a better delay than the one guaranteed by the node segment, \ie $d_1^{max}(P^*_2(x_0, x_i))$. Otherwise, the subpath exhibits a better delay than some ECMP path and must thus be encoded more precisely through additional segments.

Once one of these conditions is not met anymore, the longest prefix of $p$ encodable by a single segment is found, and the algorithm returns. 
By following these steps, Alg.~\ref{algo:encode} returns a segment list that strongly encodes the path $p$ given as input, as shown in Lemma~\ref{lem:encstr}.

\begin{Lemma}\label{lem:encstr}
    Let $S = \textsc{encode}(p)$. Then, $S$ strongly encodes $p$.
    \begin{IEEEproof}
        Any segment $S_i$ respects the conditions of strong encoding, as defined in Def.~\ref{def:encoding}.

        \begin{itemize}
            \item  Notice from Alg.~\ref{algo:1SLP} that all segments $S_i \in S$ are necessarily equal to $(t, s_i, s_{i+1})$ with $s_i \in p$ and $s_{i+1} \in p$ (Line~\ref{algo:enc:return1}, ~\ref{algo:enc:return2}, ~\ref{algo:enc:return3}). \\
            
            \item  If $S_i = (Adj, s_i, s_{i+1})$, then  $(s_i, s_{i+1}) \in p$ following Alg.~\ref{algo:encode},Line~\ref{algo:enc:return1}.\\
            
            \item Finally, if $S_i = (Node, s_i, s_{i+1})$, then each edge $e \in p_{[s_i, s_{i+1}]}$ belongs to $Dag_{[s_i, s_{i+1}]}$  meaning that $p_{[s_i, s_{i+1}]} \in P^*_2(s_i, s_{i+1})$ (following Alg.~\ref{algo:encode}, Line~\ref{test2}). Thus, by definition, $d_2(p_{[s_i, s_{i+1}]}) = d_2^{SR}(Node, s_i, s_{i+1})$.
        
            In addition, $d_1(p_{[s_i, s_{i+1}]}) \geq d_1^{SR}(Node, s_i, s_{i+1})$  (Line~\ref{test2}). Consequently, $d(p_{[s_i, s_{i+1}]})$ is dominated by $d^{SR}(S_i)$, following the definition of $d^{SR}$. \\
    
            Consequently, $S$ strongly encodes $p$, as per Def.~\ref{def:encoding}.
        \end{itemize}
        
    \end{IEEEproof}
\end{Lemma}

Furthermore, we can show that the segment list returned by \textsc{encode} encodes strongly the path given as input in the minimal number of segments.


\begin{Lemma}\label{lem:encode}    
    Let $S$ be a segment list that strongly  encodes $p$. Then, $|S| \geq |$\textsc{encode}($p$)$|$, \ie \textsc{encode} finds the minimal strong encoding of $p$.

    \begin{IEEEproof}
        Let us consider two segment lists $S = ((S_i)_{0 \leq i \leq l-1})$ and $S' = ((S'_i)_{0 \leq i \leq l'-1})$, both encoding $p$. Let $S' = \textsc{encode}(p)$ (\ie $S'$ is the result of Alg.~\ref{algo:encode}).\\
      
            \noindent
        For the sake of contradiction, let us assume that $l < l'$.
        Then, at some point, a segment $S_k$ encoded more of $p$ than $S'k$.

        Recall that, per definition of strong encoding,  $s_i \in p$.Then, there must exist $k$, $0 \leq k \leq l-1$, such that 
        \begin{enumerate}
          \itemsep0em
          \item $s_k$ appears before, or at the same place as $s'_k$ in path $p$
          \item $s_{k+1}$ appears strictly after $s'_{k+1}$ in path $p$.\\
        \end{enumerate}
      
        \noindent
        Let us start by considering that $s_k = s'_k$. Then, 2. contradicts with the fact that $S'_k$ is a path encoding the longest prefix of $p$ (recall that $S_k'$ is the output of procedure 1SegLongestPrefix on $s_k'$).\\
      
        \noindent
        Otherwise, $s_k$ appears strictly before $s'_k$ in path $p$. Notice that $S_k$ is then necessarily a node segment, as it encodes more than an edge. Following the definition of strong encoding, $p_{[s_k, s_{k+1}]} \in P^*_2(s_k, s_{k+1})$. Furthermore, as $p_{[s'_k, s_{k+1}]}$ is a subpath of $p_{[s_k, s_{k+1}]}$, $p_{[s'_k, s_{k+1}]}$ is a shortest path, following the subpath optimality property. Thus, we have 

        \[
          (i)~ p_{\left[s_k', s_{k+1}\right]} \in P^*_2(s'_k, s_{k+1})
        \] 

       When then have to prove that  
        
        \[
        (ii)~ d(p_{\left[s_k', s_{k+1}\right]})~ \text{is dominated by} ~   d^{SR}(s'_k, s_{k+1}). 
        \]
        
        Recall from Remark~\ref{rem:strenc} that $(ii)$ is equivalent to showing that $d(p_{\left[s_k', s_{k+1}\right]}) = d^{SR}(Node, s_k', s_{k+1})$. We show that this equality does indeed both for both $M_1$ and $M_2$.

        \begin{enumerate}
            \item It follows naturally from $(i)$ and the definition of $d^{SR}$ that $d_2(p_{\left[s_k', s_{k+1}\right]}) = d^{SR}_2(Node, s_k', s_{k+1})$.
            
            \item By definition of $d^{SR}$, $d_1(p_{\left[s'_k, s_{k+1}\right]}) \leq d^{SR}_1(Node, s'_k, s_{k+1})$. 
            
            Let us suppose, for the sake of contradiction, that $d_1(p_{\left[s_k', s_{k+1}\right]}) < d^{SR}_1(Node,s'_k, s_{k+1})$. Then, there exists $p' \in P_2^*(s'_k, s_{k+1})$ such that $d_1(p') > d_1(p_{\left[s_k', s_{k+1}\right]})$. Then, the path $p_{\left[s_k, s'_k\right]} \oplus p'$ is a shortest path from $s_k$ to $s_{k+1}$ (as $d_2(p') = d_2(p_{\left[s_k', s_{k+1}\right]}) = d^{SR}_2(Node, s_k', s_{k+1})$) and     
            $d_1(p_{\left[s_k, s'_k\right]} \oplus p') > d_1(p_{\left[s_k, s_{k+1}\right]})$. Consequently, we have $d^{SR}_1(Node, s_k, s_{k+1}) \geq d_1(p') > d_1(p_{\left[s_k, s_{k+1}\right]})$ (by definition of $d^{SR}$). Thus, as $d^{SR}(Node,s_k, s_{k+1})$ does not dominate $d(p_{\left[s_k, s_{k+1}\right]})$, $(Node,s_k, s_{k+1})$ does not encode $p_{\left[s_k, s_{k+1}\right]}$, which contradicts the definition of $S$. 
            
            We can then deduce that $d_1(p_{\left[s_k', s_{k+1}\right]}) = d^{SR}_1(Node,s'_k, s_{k+1})$.\\
        \end{enumerate}

        Given that $(i)$ and $(ii)$ must be true, $(Node, s'_k, s_{k+1})$ encodes $p_{\left[s'_k, s_{k+1}\right]}$, which contradicts the fact that $S'_k = (t, s'_k, s'_{k+1})$ encodes a longest prefix, as $s_{k+1}$ appears after $s'_{k+1}$ in $p$.      
      \end{IEEEproof}
\end{Lemma}



Such a conversion algorithm must be called repeatedly when exploring the graph. Indeed, simply solving DCLC and then converting the non-dominated path to a segment list is not sufficient. For example, the DCLC path returned may require more than MSD segments to encode. Consequently, the number of segments necessary to encode a path must be maintained at each extension, to maintain the entire 3D Pareto front (considering segments, delay, and cost) and ensure finding the solution to DCLC-SR. 

Considering this, we further optimize our encoding scheme. Note that the checks at Line~\ref{test1} and ~\ref{test2} can be performed efficiently through the SR graph when keeping only the edges representing node segments. Indeed, the weight of an edge within this SR graph corresponds to the distance of the associated segment. Thus, checking whether a path $p(u,v)$ can be encoded through a node segment can be done by matching its distance with the weight of the edge $w(u,v)$ with the SR Graph, \ie $d^{SR}(Node,u , v)$.


More precisely, one may check if a path $p(u,v)$ is an ECMP path by checking whether it possesses the best cost from $u$ to $v$, \ie if its cost is equal to $d^{SR}_2(Node,u,v)$ (\ie $w_2(u,v)$ in the SR Graph). Furthermore, checking whether a path $p(u,v)$ does not possess a better delay than other ECMP paths can be done by checking whether its delay is equal to $d^{SR}_1(Node, u, v)$. 

Furthermore, while Alg.~\ref{algo:encode} and ~\ref{algo:1SLP} assume that the whole path is given as input, the latter can be easily modified to consider paths edges by edges and correctly update the corresponding segment lists to encompass each new edge, instead of re-considering the entire path.

From these observations, we derive a new algorithm able to strongly encode paths in segment lists \emph{during} the exploration of said path while relying on efficient tests performed via the SR Graph.





\begin{algorithm}
    \footnotesize
    \caption{ \footnotesize \lca($S$, $e=(u,v)$)}\label{algo:lca}
    $(t,s,u)$ = $S_{l-1}$\\
  
    \If{$S = [~]$}{
        $t = None$\\
        $s = u$\\
    }
    %\If{$t = Node$ \textbf{and} $d_2(S) + w_2(e) = w^{G'}(s,v)$ \textbf{and} $w^{G'}_1(s, v) \leq w^{G'}_1(s,u) + w_1(e)$}{\label{lca:line1}
    
    \If{$t = Node$ \textbf{and} $d^{SR}(S_{l-1}) + w(e) = d^{SR}(Node, s, v)$}{\label{lca:line1}
    $S_{l-1} = (t, s, v)$\\
    \Return $S$\label{algo:lca:return2}\\
    }

    \If{$w(e) \neq d^{SR}(Node, s, v)$} {\label{lca:line5}
    $S$.push($(Adj, u, v)$)\\
    \Return $S$\label{algo:lca:return1}\\
}
   
    $S$.push($(Node, u, v)$)\\
    \Return $S$\label{algo:lca:return3}\\  
\end{algorithm}


\lca (Alg.~\ref{algo:lca}) takes as input a segment list strongly encoding a path $p$, and an edge $e$. It then returns a new segment list, strongly encoding $p \oplus e$. \lca follows the same general idea as Alg.~\ref{algo:encode} and ~\ref{algo:1SLP}, \ie encoding the longest possible prefix through a single segment. 

More precisely, \lca starts by retrieving the last segment of the segment list $S_{l-1} = (t,s,u)$. It then checks if this segment can be updated to $(t,s,v)$ to encompass the new edge $e$. Since an adjacency segment may only encode one segment, updating $(t,s,u)$ to $(t,s,v)$ is only possible if $t = Node$. To ensure that the new, extended path is strongly encoded by $(Node,s,v)$, the distance of the path is matched against the distance of said node segment (see Line~\ref{lca:line1}). The last segment is then modified accordingly. 

Otherwise, a new segment is necessarily required. Line~\ref{lca:line5} checks whether this new segment should be an adjacency (\ie by matching the weight of $e$ against the node segment $(Node, u,v)$) or a node segment. The new segment is then pushed onto $S$, which is returned. We now show that relying on \lca allows computing the same segment lists as \textsc{encode}.

To do so, we will consider a simple wrapper to the \lca function, which calls \lca iteratively on each edge of a path and returns the resulting segment list. 


\begin{algorithm}
    \footnotesize
    \caption{ \footnotesize \textsc{lca\_wrapper}($p = (x_0, x_1)\dots(x_{l-1}, x_l)$)}\label{algo:lcawrapper}
    $S = (Node, x_0, x_0)$\\
    \For{$e \in p$}{
        $S = \lca(S, e)$
    }
    \Return $S$\\  
\end{algorithm}
   

\begin{Lemma}\label{lem:lcaencode}
    Let $p$ be a path. Then, \textsc{lca\_wrapper}($p$) $=$ \textsc{encode}($p$). 
    \begin{IEEEproof}

    Let $S^{lca}$ be the segment list obtained when calling \textsc{lca\_wrapper} with a given path $p$ as argument, and $S^{enc}$ the segment list obtained when calling \textsc{encode} $p$ as argument. \\

    We will prove by induction that, when encoding a path $p$ of $n$ edges, $S^{lca} = S^{enc}$.\\

    \underline{Base case (n = 1)}\\
    
    When $n = 1$, the path is composed of a single edge $e = (u,v)$.  Any encoding segment will thus necessarily be equal to $S = (t, u, v)$. Consequently, it suffices to show that $t^{lca}_0 =  t^{enc}_0$. 

   Suppose that $t^{lca}_0 = Adj$. By following Alg.~\ref{algo:lca}, this implies $w(e) \neq w^{G'}(u,v)$, \ie $w(e) \neq d^{SR}(Node,u,v)$, by definition of the SR graph and $d^{SR}$. If $w(e) \neq w^{G'}(u,v)$, either 
   \begin{enumerate}
    \item $ w_1(e) < d_1^{SR}(Node, u, v)$, \ie $w_1(e) < d_1^{max}(P^*_2(u, v))$
    \item $ w_2(e) > d_2^{SR}(Node, u,v)$ \ie $w_2(e) > d_2^*(u,v)$ and so $e \notin Dag_{\left[u,v\right]}$, by definition of $d^{SR}$.
   \end{enumerate}

  Consequently, given Line~\ref{test1} of Alg.~\ref{algo:1SLP}, $t^{enc}_0 = Adj$. Thus, $t^{lca}_0 = Adj$ implies that $t^{enc}_0 = Adj$.

   If $t^{lca} = Node$, then $w(e) = d^{SR}(Node,u,v)$. Thus, $w_2(e) = d_2^*(u,v)$, meaning that $(u,v) \in Dag_{\left[u,v\right]}$, and $w_1(e) = d_1^{max}(P^*_2(u, v))$. Consequently, according to Line~\ref{test1} of Alg.~\ref{algo:1SLP}, $t^{enc}_0 = Node$. Thus, $t^{lca}_0 = Node$ implies that $t^{enc}_0 = Node$. The property then holds for $n = 1$. \\

   \underline{Inductive hypothesis}\\

   Let $k$ be given and suppose that the property remains true for $n = k$, \ie that \textsc{encode}($p$)=\textsc{lca\_wrapper}($p$) for any $p$ of $n$ edge. We show that this remains true when considering a path $p' = p \oplus e$.\\

   \underline{Inductive step}\\

  
   \textbf{When encoding $p+e$, both segment lists may gain one or zero additional segment.}\\

   

   Let $p = (x_0, x_1)\dots(x_{n-1}, x_{n})$ be a path of $n$ edge. By hypothesis, $S^{enc} =$\textsc{encode}($p$) is equal to $S^{lca} =$\textsc{lca\_wrapper}($p$) and both segment lists possess the same number of segments, \ie $l^{enc} = l ^{lca} = l$. Consequently, $S^{enc}_{[0, l-2]} = S^{lca}_{[0, l-2]}$.

   Let us consider the path $p' = p \oplus e$ of $n+1$ edges, with $e=(x_n, x_{n+1})$. Let $S^{enc'} =$\textsc{encode}($p'$) and $S^{lca'} =$\textsc{lca\_wrapper}($p'$). Note that both $S^{enc'}$ and $S^{lca'}$ have at most $l+1$ segment. Indeed, if $l^{enc'} > l+1$, then there exists a segment lists $S = S^{enc} \oplus (Adj, x_n, x_{n+1})$ which strongly encodes $p'$ in $l+1$ segments, which contradicts Lemma~\ref{lem:encode}. Furthermore, following Alg.~\ref{algo:lca}, a new edge $e$ may either add a single segment (Line~\ref{algo:lca:return1} and ~\ref{algo:lca:return3}) or leave the number of segments unchanged (Line~\ref{algo:lca:return2}). Thus, we have $l \leq l^{enc'} \leq l+1$ and $l \leq l^{lca'} \leq l+1$.\\

   \textbf{As $e$ may only impact the last segment, showing that both algorithms choose the same last(s) segment(s) is sufficient.}\\
   
   Clearly from the pseudo-code of the algorithm, the edge $e$ can only impact the last segment of $S^{enc'}$ and $S^{lca'}$ (\ie the $l^{th}$ or $l+1^{th}$ segment). 

   More precisely, considering $e$ may either add a new segment to the list, or change the last segment. Previous segment are not impacted. 
   
   Thus, we have at least $S^{enc'}_{[0, l-2]} = S^{enc}_{[0, l-2]}$ and $S^{lca'}_{[0, l-2]} = S^{lca}_{[0, l-2]}$. Recall that $S^{enc}_{[0, l-2]} = S^{lca}_{[0, l-2]}$. 
  
   Consequently, $S^{lca'}_{[0, l-2]} = S^{enc'}_{[0, l-2]}$. It is thus sufficient to show that the last(s) segment(s) of $S^{lca'}$ and $S^{enc'}$ are identical.\\


   \textbf{When $l^{enc'} = l$, then both \textsc{encode}($p \oplus e$) and \textsc{lca\_wrapper}($p \oplus e$) output the same segment list.}\\



   Since we already know that $S^{lca'}_{[0, l-2]} = S^{enc'}_{[0, l-2]}$, it is sufficient to show that $S^{lca'}_{l-1} = S^{enc'}_{l-1}$ to prove that $S^{enc'} = S^{lca'}$, as both will then encode the entirety of $p'$ and be of size $l$. By hypothesis, we know that $S^{lca}_{l-1} = (Node, x_i, x_{n}$) (recall that $S^{lca}_{l-1} = S^{enc}_{l-1} = $\textsc{encode}($p$)). There is thus only one possibility : \textsc{encode} chose to update its last (node) segment to encompass the new edge $e$. We will now show that in this case, \lca would follow the same behavior.
 
   Let us suppose that $l^{enc'} = l$. Following Alg.~\ref{algo:encode}, that means that the ultimate call to \textsc{1SegLongestPrefix} reached Line~\ref{algo:enc:return3}, meaning that $S^{enc}_{l-1} = (Node, s_{l-1}, x_{n})$ and $S^{enc'}_{l-1} = (Node, s_{l-1}, x_{n+1})$. We then know that $e \in Dag_{[s_{l-1}, x_{n+1}]}$ and $d_1(p_{[s_{l-1}, x_{n+1}]}) \geq d_1^{SR}(Node,x_i, x_{n+1})$.  Given that $e \in Dag_{[x_i, x_{n+1}]}$, then $d^{SR}_2(S^{lca}_{l-1}) + w_2(e) =  d^*_2(x_i, x_{n+1}) =  d^{SR}(x_i,x_{n+1})$. 

Furthermore, as $d_1(p_{[x_i, x_{n+1}]}) \geq d_1^{SR}(Node,x_i, x_{n+1})$, we know that $d_1(p_{[x_i, x_{n}]}) + w_1(e) = d_1^{SR}(Node,x_i, x_{n+1})$. Since $(Node, x_i, x_n)$ encodes $p_{[x_i, x_{n}]}$, it follows that $d_1^{SR}(p_{[x_i, x_{n}]}) + w_1(e) = d_1^{SR}(Node,x_i, x_{n+1})$. Consequently, from both equalities, we know that Line~\ref{lca:line1} is verified and that \lca also changes the last segment to $(Node, x_i, x_{n+1})$. No edges are left to consider.\\

\textbf{When $l^{enc'} = l+1$, then both \textsc{encode}($p \oplus e$) and \textsc{lca\_wrapper}($p \oplus e$) output the same segment list.}\\

Let us now suppose that $l^{enc'} = l+1$. Since the last segment results from the addition of $e$ to the path, said segment necessarily encodes $e$. Thus, $S^{enc'}_{l}$ may take only two values : either $S^{enc'}_{l} = (Node, x_n, x_{n+1})$ or $S^{enc'}_{l} = (Adj, x_n, x_{n+1})$. Consequently, the penultimate segment of $S^{enc'}$ may also only take two values : (i) $(Node, s_{l-1}, x_n)$ or (ii) $(Adj, x_{n-1}, x_n)$.


 

\begin{enumerate}[label=(\roman*)]
    \item \textit{If the penultimate segment of $S^{enc'}$, \ie $S^{enc'}_{l-1}$ is a node segment, both \textsc{encode}($p \oplus e$) and \textsc{lca\_wrapper}($p \oplus e$) output the same segment list}\\
    
    Here, we have $S^{enc'}_{l-1} = (Node, s_{l-1}, x_n)$. Since $e$ only added a new segment to the list, we know that $S^{enc'}_{l-1} = S^{enc}_{l-1}$, and so that $S^{enc'}_{l-1} = S^{enc}_{l-1} = S^{lca}_{l-1}$. Thus, $S^{lca}_{l-1} = (Node, s_{l-1}, x_n)$.

    While both segment lists end with the same node segment, this does not mean that they remain the same after considering $e$, \ie it does not ensure that $S^{enc'}_{l-1} = S^{lca'}_{l-1}$. Indeed, while we know that \textsc{encode} chose to add a new segment to the segment list (since $l^{enc'} = l+1$) and leave $S^{enc'}_{l-1}$ unchanged, \lca could have chosen to update the node segment $S^{lca}_{l-1}$ to encompass $e$, and not add any new segment after that. Thus, we have to prove that if \textsc{encode} chose to add a new node or adjacency segment after $S^{enc'}_{l-1} =  S^{lca}_{l-1}$, so did \lca. \\

    
    If $S^{enc'}_{l} = (Node, x_{n}, x_{n+1})$, then two possible conditions could have been verified for \textsc{encode} to add this segment. 

    Either, $(x_{n}, x_{n+1}) \notin Dag_{[s^{enc'}_{l-1}, x_{n+1}]}$, in which case $p_{[s^{enc}_{l-1}, x_{n-1}]} \oplus (x_{n-1}, x_n)$ is not a shortest path. Since $d^{SR}(S_{l-1}) = p_{[s^{enc}_{l-1}, x_{n}]}$ by definition, 
    then $d^{SR}(S_{l-1}) + (x_{n}, x_{n+1}) \neq d^{SR}_{Node, s^{enc}_{l-1}, x_{n+1}}$, meaning that Line~\ref{lca:line1} of \lca is not verified.

    Or, $d^1(p_{[s^{enc}_{l-1}, x_{n+1}]}) < d_1^{SR}(Node, s^{enc}_{l-1}, x_{n+1})$. In this case, $d_1(p_{[s^{enc}_{l-1}, x_{n}]}) + w_1(e) < d_1^{SR}(Node, s^{enc}_{l-1}, x_{n+1})$, meaning that $d_1^{SR}(Node, s^{enc}_{l-1}, x_n) + w_1(e) < d_1^{SR}(Node, s^{enc}_{l-1}, x_{n+1})$, \ie that $d^{SR}(S_{l-1})+ w_1(e) < d_1^{SR}(Node, s^{enc}_{l-1}, x_{n+1})$. Line~\ref{lca:line1} of \lca is consequently still not verified. 

    Finally, we know that $(x_{n}, x_{n+1}) \in Dag_{[x_{n}, x_{n+1}]}$  and $w_1(x_{n}, x_{n+1}) < d_1^{SR}(Node, x_{n}, x_{n+1})$ (else \textsc{1SegLongestPrefix} would have returned an adjacency segment). Thus, clearly, we have $w_2(x_n, x_{n+1}) = d_2^*(x_{n}, x_{n+1}) = d_2^{SR}(Node,x_{n}, x_{n+1})$. Furthermore, we know that $w_1(x_{n}, x_{n+1}) \geq d^{SR}_1(Node, x_{n}, x_{n+1})$ for the same reason. Thus, $w_1(x_{n}, x_{n+1}) = d^{SR}_1(Node, x_{n}, x_{n+1})$, per definition of $d^{SR}$. Consequently, $w_(x_{n1}, x_{n+1}) = d^{SR}(Node, x_{n}, x_{n+1})$, meaning that Line~\ref{lca:line5} is not verified. 

Consequently, if $S^{enc'}_{l} = (Node, x_{n}, x_{n+1})$, then $S^{lca'}_{l} = (Node, x_{n}, x_{n+1})$.\\

If $S^{enc'}_{l} = (Adj, x_{n}, x_{n+1})$, then two conditions had to be verified for \textsc{encode} to add this segment. First, $(x_{n}, x_{n+1}) \notin Dag_{[x_{n}, x_{n+1}]}$  and second, $w_1(x_{n}, x_{n+1})  < d_1^{SR}(Node, x_{n}, x_{n+1})$. 

Since $(x_{n}, x_{n+1}) \notin Dag_{[x_{n}, x_{n+1}]}$, it follows than $p_{[x_{l-1}, x_{n}]} \oplus  (x_{n}, x_{n+1})$ is not a shortest path from $x_{l-1}$ to $x_{n}$, and so that $d_2(p_{[x_{l-1}, x_{n}]}) +  w_2(x_{n}, x_{n+1}) \neq d^{SR}(Node, x_{l-1}, x_{n})$ by definition of $d^{SR}$. Since $S^{lca}_{l-1}$ encodes $p_{[x_{l-1}, x_{n}]}$ (recall that $S^{enc'}_{l-1} = (Node, x_{l-1}, x_{n}) = S^{lca}_{l-1}$), then $d(p_{[x_{l-1}, x_{n}]}) = d^{SR}(S^{lca}_{l-1})$, meaning that $d^{SR}(S^{lca}_{l-1}) + w_2(x_{n}, x_{n+1}) \neq d^{SR}(Node, x_{l-1}, x_{n})$. Thus, Line~\ref{lca:line1} of \lca is not verified.

Since $w_1(x_{n}, x_{n+1})  < d_1^{SR}(Node, x_{n}, x_{n+1})$, then $w(x_{n}, x_{n+1}) \neq d^{SR}(Node, x_{n}, x_{n+1})$, meaning that Line~\ref{lca:line5} of \lca is verified, and that \lca also adds $(Adj, x_{n}, x_{n+1})$ to its segment list.



\item \textit{If the penultimate segment is an adjacency segment, both \textsc{encode}($p \oplus e$) and lca\_wrapper($p \oplus e$) output the same segment list}\\

Similarly to the previous case, we necessarily have $S^{enc'}_{[0,l-1]} = S^{lca'}_{[0,l-1]} = (Adj, x_{n-1}, x_{n})$. However, in this case, both algorithms have to add another segment to the list during the next step, as an adjacency segment can only encompass one edge. 

Furthermore, note that when encoding the last edge $e = (x_n, x_{n+1})$, \lca will thus consider $s =  x_n$, $t = Adj$ and thus behave exactly as if encoding a path of a single edge $p = (x_n, x_{n+1})$. Similarly, the last call of \textsc{1SegLongestPrefix}, by design, will behave exactly like if encoding a path $p = (x_n, x_{n+1})$. Consequently, the argument used for the case $n=1$ is identical and holds.

\end{enumerate}



\textbf{Thus, we have \textsc{encode}($p+e$) = \textsc{lca\_wrapper}($p+e$), meaning that \textsc{encode}($p$) = \textsc{lca\_wrapper}($p$) for all $p$.}
    
    \end{IEEEproof}
\end{Lemma}

Lemma~\ref{lem:lcastr} follows naturally from Lemma~\ref{lem:lcaencode}. 

\begin{Lemma}\label{lem:lcastr}
\lca allows computing the minimal strong encoding of any given path $p$.
\end{Lemma}

As long as the segment lists encoding the paths being explored are maintained, \lca may be fitted onto any shortest path computation algorithm to encode paths into segment lists that ensure that their distance is respected. The associated overhead is negligible, as the required checks can be performed very efficiently if the SR graph was computed beforehand. \\

However, simply relying on \lca to track the size of the segment lists is not sufficient by itself to solve DCLC-SR. Because of the peculiarities of the segment metric, some \emph{dominated} paths must be maintained and extended to retrieve the entirety of the three-dimensional Pareto front.

\subsection{Keeping (some) dominated paths}

Although the algorithms presented in the previous section allow finding the minimal number of segments to strongly encode a path, other modifications are required to correctly consider the number of segments as a new dimension when computing paths.


The notion of dominance is central to most DCLC schemes to limit the number of distances to extend. The standard definition of dominance is straightforward: a distance toward a node $u$ is dominated if all the components of its weight vector are worse than or equal to another distance towards the same node (see Section~\ref{sec:multi-metric-path-computation}). Dominated distances can usually be ignored, as they cannot lead to better distances overall. Indeed, as both distances may benefit from the same edges onwards, there is no way for the dominated distance to improve upon the non-dominated one. 


This simple property does not behave in the same fashion when considering the number of segments as a new dimension of the paths' distance. Indeed, extending a distance by an edge $(u,v)$ may or may not cost an additional segment, depending on the actual \emph{path} used to reach $u$. As distances may be extended with no impact on the number of segments, distances that seem dominated may become non-dominated later on, or may even be the only feasible distances at the end of the exploration. \\



\begin{figure}
    \centering
    \begin{subfigure}{.45\textwidth}
      \centering
      \includegraphics[scale=0.78]{./figures/COMEBACKREAL.pdf}
      \caption{\textsc{comeback} gadget.}\label{fig:comback}
    \end{subfigure}\hfill
    \begin{subfigure}{.50\textwidth}
      \centering
      \includegraphics[scale=0.7]{./figures/UNDERDAGREAL.pdf}
      \caption{\textsc{underdag} gadget.}\label{fig:underdag}
    \end{subfigure}
    \caption{Figures illustrating the peculiarities of the number of segment metric.}
    \label{fig:lcagadgets}
\end{figure}


These peculiarities are illustrated in Fig.~\ref{fig:lcagadgets}. Let us consider the \textsc{comeback} gadget. Two delay-cost vectors $(d_1;d_2)$ exist to reach $u$ from $s$ : $(1;1)$ and $(1;100)$. Both can be encoded with a single node ($(Adj, s, u)$ and $(Node, s, u)$ respectively), leading to the distances $d(s,u) = (1;1;1)$  and $d'(s,u) = (1;1;100)$, where the first component $d_0$ is the number of segments. Note that following the standard definition of dominance, $d'(s,u)$ is dominated. 

Both $d'$ and $d$ can be extended by $(u,v)$, leading to the delay-cost vector $(2;2)$ and $(2;101)$. However, while the vector $(2;2)$ requires an additional node segment to be encoded (following the adjacency segment), the vector $(2;101)$ remains encodable through a single node segment $(Node, s, v)$. Thus, upon extension, the obtained distances are $d(s,v) = (2;1;1)$ and $d'(s,v) = (1;1;100)$. 

While resulting from the extension of a dominated distance, $d'(s,v)$ is non-dominated (and the only feasible distance when considering a strict $c_0$ constraint of 1). 

In the \textsc{comeback} gadget, this effect results from the fact that  an adjacency segment may only encode a single link. Hence, the following edges to encode will necessarily require additional segments. On the opposite, a node segment may encode any path lying within the shortest path DAG of the current source. Thus, as long as the next edges remain within said DAG, additional segments may not be required (depending on the weight of said edges). Rather, the current node segment may simply be updated to encode the following edges. \\


However, this effect may also occur even if both segment lists end with a node segment. This is illustrated by the \textsc{underdag} gadget. Let us consider the delay-cost vectors from $s$ to $u$ $(2;2)$ and $(3;2)$, from the paths $p(s,u) = (s_1, a),(a,u)$ and $p'(s,u) = (s_1,b),(b,u)$ respectively. These distances and paths can be encoded by the segments lists $S = (Adj, s_1, a) | (Node, a, u)$ and $S' = (Adj, s_1, b) | (Node, b, u)$ respectively. Thus, their distances are $d = (2;2;2)$ and $d' =(3;2;2)$. Note that $d'$ is dominated by $d$, and that both $S$ and $S'$ are composed of segments of the same type. 

However, notice that the edge $(u,v)$ lies within the shortest path DAG of $b$. Hence, the last segment of $S'$, $(Node, b, u)$, may simply be updated to $(Node, b, v)$ to encompass $(u,v)$.  On the contrary, the edge $(u,v)$ does not lie within the shortest path DAG of $a$. Thus, the last segment of $S$, $(Node, a, u)$ may not be updated to encompass $(u,v)$, and a new segment is required. Consequently, once updated, the distances to $v$ are $d = (4;3;3)$ and $d' = (5;3;2)$. Once again, the non-dominated distance $d'$ results from the extension of a dominated distance.\\



From these observations, we derive and formally define the \emph{strong dominance} relation. Strong dominance encompasses the peculiarities of the new metric when considering strong encoding, and should thus be followed when relying on \lca to correctly solve DCLC-SR.

\begin{Definition}[Strong dominance]\label{def:sreff}
    Let $d$ and $d'$ be two distances encoding two paths $p$ and $p'$ from  $x_0$ to $x_k$, composed of three components $d_0, d_1 , d_2$, representing their number of segments, delay and cost respectively. Let $S = (t_i, s_i, s_{i+1})_{0 \leq i\leq l-1}$ and $S' = (t'_i, s'_i, s'_{i+1})_{0 \leq i \leq l'-1}$ be their respective (encoding) segment lists. \\
    
    \noindent
    The segment list $S$ is strongly dominated by $S'$ if it is dominated by $d'$ (as per Def.~\ref{def:dominance}), \emph{and} if either :

    \begin{enumerate}
        \itemsep0em
        \item $d_0 > d'_0$, or
        \item $t_{l-1} = t'_{l-1} \wedge d^{SR}(Node, s_{l-1}, s'_{l'-1}) + d^{SR}(Node, s'_{l'-1}, x_k)  = d^{SR}(Node, s_{l-1}, x_k)$
        % \item $s_{l-1} = s'_{l-1} \wedge t_{l-1} = t'_{l-1}$ 
        % \item $s'_{l-1} \in Dag_{[s_{l-1}, x_k]} \wedge t_{l-1} = t'_{l-1}$ 
      \end{enumerate}    

\end{Definition}


While the importance of the conditions within Def.~\ref{def:sreff} are thoroughly detailed and leveraged within the following proofs, we will first describe their impact informally. Intuitively, if $S$ is dominated by $S'$, it will necessarily (by definition) remain dominated regarding its cost and delay, as both distances may be extended by the same edges, which have the same impact on both metrics. The additional conditions thus focus on the number of segment, which may evolve differently despite being extended by the same edge (as seen in Fig~\ref{fig:lcagadgets}), and ensures that $S$ remains dominated when considering this metric as well despite its odd behavior. 

Less formally, we state that a segment list $S$ is strongly dominated by $S'$ if it is dominated by $S'$, and if \emph{one} of two conditions is verified. 

The first condition is that the number of segments of $S$ is strictly superior to that of $S'$. Otherwise, as the number of segments does not necessarily increase in a strictly monotonous fashion, it is possible for $d_0$ to become smaller than $d'_0$ (as we have seen in Fig.~\ref{fig:lcagadgets}). However, we will prove that such a case (where $S$ does not require an additional segment while $S'$ does) may only happen once in a row. Hence, ensuring that $d_0 > d'_0$ is sufficient.

The second condition is perhaps less intuitive. Intuitively, the condition ensures that if $S$ does not require another segment to encode an additional edge, neither does $S'$, meaning that $S$ is bound to remain dominated by $S'$.\\

Maintaining and extending only distances that are not strongly dominated allows pruning some distances from further exploration without compromising the integrity of the returned Pareto front, as stated and proved in Lemma~\ref{lem:extdom}.


\begin{Lemma}\label{lem:extdom}
    A segment list that is strongly dominated remains strongly dominated after being extended. 
    \begin{IEEEproof}

%    We will prove this Lemma by induction. 

    Let $S$ be a segment list, and $d$ the associated distance.  Let $S$ be strongly dominated. 

    Since $S$ is strongly dominated, there exists a segment list $S'$ (having a distance $d'$) such that $S$ is dominated by $S'$, and either (i) $t_{l-1} = t'_{l-1} \wedge d^{SR}(Node, s_{l-1}, s'_{l'-1}) + d^{SR}(Node, s'_{l'-1}, xn)  = d^{SR}(Node, s_{l-1}, x_n)$ or (ii) $d_0 > d'_0$. Let us denote $S^{+1}$ the segment list $S$ once extended by an additional edge $(u,v)$, and $d^{+1}$ the associated distance.\\

    \textbf{If $d$ is dominated by $d'$ and $t_{l-1} = t'_{l-1} \wedge d^{SR}(Node, s_{l-1}, s'_{l'-1}) + d^{SR}(Node, s'_{l'-1}, x_n)  = d^{SR}(Node, s_{l-1}, x_n)$, $S^{+1}$ is strongly dominated when extended by an edge $(u,v)$.}\\


    Clearly, when extending by the same edge $e = (u,v)$, the cost and the delay of $d$ and $d'$ evolves in the same fashion. We thus need to ensure that $d^{+1}_0 \geq d'^{+1}_0$, and that (i) or (ii) is still verified.\\

   \textit{$d$ remains dominated}\\

   Note that when extending a distance and relying on the conversions schemes aforementioned, the number of segments may either stay the same or increase by one. The distances $d_0$ and $d'_0$ may thus evolve in four different fashion: either both increase by one, none increase by one, or one of them increases by one. We will refer to these cases as +1/+1 (both gain one segment), +0/+0 (both remain identical), +1/+0 (only $d_0$ gains a segment when extended) and +0/+1 (only $d'_0$ gains a segment when extended).

   Note that in all cases but one, the dominance relationship remains unchanged. Solely the +0/+1 case may render $d^{+1}_0$ non-dominated. However, recall that we mentioned earlier in this section that condition (i) ensures that if $S$ does not require an additional segment, neither does $S'$, meaning that this case may not occur if (i) is verified, as we will now show.

   If $S$ did not require an additional segment, then $S_{l-1}$ is a node segment, meaning that $S'_{l'-1}$ is a node segment as well (since (i) holds).    
   
   Furthermore, this means that $d_2^{SR}(S_{l-1}) + w_2(u,v) = d_2^{SR}(Node, s^n_{l-1}, v)$. Thus, a shortest path from $s_{l-1}$ to $v$ goes through $u$. Since a shortest path is necessarily composed of shortest subpaths, we have $d^{SR}_2(s_{l-1}, v) = d^{SR}_2(s^n_{l-1}, u) + w(u,v)$. Since (i) hold, we have $d^{SR}_2(s_{l-1}, u) = d^{SR}_2(s_{l-1}, s'_{l'-1}) + d^{SR}_2(s'_{l'-1}, u)$. It follows than 
   
   \begin{equation}\label{eq:1}
    d^{SR}_2(s_{l-1}, v) =  d^{SR}_2(s_{l-1}, s'_{l'-1}) + d^{SR}_2(s'_{l'-1}, u) + w(u,v).
   \end{equation}
   

   Notice that the triangle inequality hold for $d_2$. Consequently, we have $d^{SR}_2(s'_{l'-1}, u) \leq d^{SR}_2(s'_{l'-1}, u) + w_2( u, v)$. Similarly, we know that $d^{SR}_2(s_{l-1}, s'_{l'-1}) + d^{SR}_2(s'_{l'-1}, v) \geq d^{SR}_2(s_{l-1}, v)$, \ie that $$d^{SR}_2(s'_{l'-1}, v) \geq d^{SR}_2(s^n_{l-1}, v) - d^{SR}_2(s_{l-1}, s'_{l'-1})$$. Coupled with Eq.~\ref{eq:1}, we can deduce that $$d^{SR}_2(s'_{l'-1}, v) \geq  d^{SR}_2(s^n_{l-1}, s'_{l'-1}) + d^{SR}_2(s'_{l'-1}, u) + w_2(u,v) - d^{SR}_2(s^n_{l-1}, s'_{l'-1})$$ And so that $d^{SR}_2(s'_{l'-1}, v) \geq d^{SR}_2(s'_{l'-1}, u) + w_2(u,v)$. Consequently, we know that $$d^{SR}_2(s'_{l'-1}, v) = d^{SR}_2(s'_{l'-1}, u) + w_2(u,v)$$.

   Furthermore, we know that $d^{SR}_1(s'_{l'-1}, v) = d^{SR}_1(s'_{l'-1}, u) + w_1(u,v)$. Let us suppose, for the sake of contradiction that $d^{SR}_1(s'_{l'-1}, v) \neq d^{SR}_1(s'_{l'-1}, u) + w_1(u,v)$. Then, as $d^{SR}_1(s'_{l'-1}, u) + w_1(u,v)$ is a shortest path, we know by definition that $d^{SR}_1(s'_{l'-1}, v) > d^{SR}_1(s'_{l'-1}, u) + w_1(u,v)$, meaning that there exist a shortest path $p$ from  $s'_{l'-1}$ to $v$ with a delay higher than $d^{SR}_1(s'_{l'-1}, u) + w_1(u,v)$. However, in this case, we would have $d^{SR}_1(s_{l-1}, v) =  d^{SR}_1(s^n_{l-1}, s'_{l'-1}) + d^{SR}_1(s'_{l'-1}, u) + w(u,v) < d^{SR}_1(s_{l-1}, s'_{l'-1}) + d_1(p)$, which contradicts the definition of  $d^{SR}_1$.\\



   Thus, for all \emph{possible} cases, $d^{+1}$ remains dominated if (i) is verified. \\

   \textit{(i) or (ii) remains verified}\\

   %$$d^{SR}(Node, s_{l-1}, s_{l-1}') + d^{SR}(Node, s_{l-1}',u) = d^{SR}(Node, s_{l-1}, u)$$

    Let us start by considering the +0/+0 case. Then, both segment lists $S^n$ and $S'$ ended with a node segment that has been updated. Let us denote $S'^{+1}$ the segment list $S'$ after being extended. Clearly, $t^{+1}_{l}$ = $t'^{+1}_{l'} = Node$. Similarly, we have $s^{+1}_{l} = s_{l-1}$ and $s'^{+1}_{l'-1} = s'_{l'-1}$. Since the last (node) segment of $S$ was updated, then we have 
    
    \begin{equation}\label{eq:A}
      d^{SR}(Node, s_{l-1}, u) + w(u,v) = d^{SR}(Node, s_{l-1}, v)
    \end{equation}

    Furthermore, as (i) was verified prior to the extension, we know that 
    
    \begin{equation}\label{eq:B}
      d^{SR}(Node, s_{l-1}, s'_{l-1}) + d^{SR}(Node, s'_{l'-1}, u) = d^{SR}(Node, s_{l-1}, u)
    \end{equation}
    
    
    It follows from Eq.~\ref{eq:A} and Eq.~\ref{eq:B} that 
    
    \begin{equation}\label{eq:C}
      d^{SR}(Node, s_{l-1}, s'_{l'-1}) + d^{SR}(Node, s'_{l'-1}, u) + w(u,v) = d^{SR}(Node, s_{l-1}, v)
    \end{equation}
    

    However, recall that $S'$ also updated its last node segment, meaning that 
    
    \begin{equation}\label{eq:D}
      d^{SR}(Node, s'_{l-1}, u) + w(u,v) = d^{SR}(Node, s'_{l'-1}, v)
    \end{equation}
    
    It follows from Eq.~\ref{eq:C} and Eq.~\ref{eq:D} that $$d^{SR}(Node, s_{l-1}, s'_{l'-1}) + d^{SR}(Node, s'_{l'-1}, v) = d^{SR}(Node, s_{l-1}, v)$$, meaning that condition (i) remains verified.

    Considering the +1/+1 case, then both segment list where either extended by one node segment $(Node,u,v)$ or one adjacency segment $(Adj, u, v)$. Clearly, if both $S$ and $S'$ require a new segment, then the edge $(u,v)$ does not lie on a shortest path from $s_{l-1}$ to $v$, or had a better delay that other shortest paths. The similar reasoning can be had regarding $s'_{l'-1}$. The choice between an adjacency and a node segment thus boils down to whether $(u,v)$ is the shortest path between $u$ and $v$ and, if it is, it possesses the highest delay among all shortest path between $u$ and $v$. Clearly, this choice does not depend on any previous segment, and both $S$ and $S'$ will be extended in the same fashion. Thus, we have $t^{+1}_{l^{+1}}$ = $t'^{+1}_{l'^{+1}} = Node$. Since $s^{+1}_{l} = s'^{+1}_{l'} = u$, then (i) clearly remains verified, as the condition translates to $d^{SR}(Node, u, u) + d^{SR}(Node, u, v) = d^{SR}(Node, u, v)$. 

   Finally, we consider the last possible case, \ie the +1/+0 case. Note that by definition, we know that $d_0 \geq d'_0$ (as $d$ is dominated by $d'$). Then, in the +1/+0 case, we necessarily have $d^{+1}_0 > d'^{+1}_0$, meaning that (ii) is verified. 

   Thus, in all cases considered above, $d$ remains dominated by $d'$ after being extended. We now prove that the same is true when (ii) is verified. \\




   \textbf{If $d$ is dominated by $d'$ and $d_0 > d'_0$, $d^{+1}$ is strongly dominated.}\\
    
    
   \textit{$d^{+1}$ remains dominated}\\

   Similarly to the previous case, we simply need to ensure that after being extended, $d^{+1}_0 \geq d'^{+1}_0$. 

   Let us consider the four possible cases. Clearly, for all possible cases +0/+0, +1/+1, +1/+0, +0/+1, we have either $d^{+1}_0 > d'^{+1}_0$ or $d^{+1}_0 = d'^{+1}_0$, meaning that $d^{+1}$ is dominated by $d'^{+1}$.\\


   \textit{(i) or (ii) remains verified}\\

   For cases +0/+0, +1/+1, +1/+0, $d^{+1}_0 > d'^{+1}_0$ clearly remains true, meaning that (ii) remains verified and that $d^{+1}_0$ remains strongly dominated. 


   Let us consider the case +0/+1. In this case, it is possible that $d^{+1}_0 = d'^{+1}_0$, meaning that (ii) would not be verified anymore. However, recall that earlier in this section, we stated that such a case may only occur once in a row. Indeed, if this case occurs, then (i) becomes verified, meaning that the +0/+1 case cannot occur at the next iteration, as proved earlier. Let us show that (i) is now indeed verified.

   In this case, we know that the last segment of $S^{+1}$ is a node segment $(Node, s^{+1}_{l - 1}, v)$, that has just been updated to encompass the edge $(u,v)$. As a node segment may only encode shortest paths (with the highest delay), we know that the edge $(u,v)$ must also be a shortest path from $u$ to $v$, and possess the maximum delay among all these shortest paths. We can than deduce that $w(u,v) =  d^{SR}(Node,u,v)$ meaning that the segment added to $S'$ is also node segment. Thus, the last segment of $S^{+1}$ and $S'^{+1}$ share the same type. 

   Furthermore, we know that $d^{SR}(Node, s_{l - 1}, u) + w(u, v) = d^{SR}(Node, s_{l - 1}, v)$. As $w(u,v) =  d^{SR}(Node,u,v)$, we know that $d^{SR}(Node, s_{l - 1}, u) + d^{SR}(Node,u,v) = d^{SR}(Node, s_{l - 1}, v)$. However, since the last segment of $S'^{+1}$ is necessarily $(Node, u,v)$, then $s'^{+1}_{l'} = u$. Furthermore, we have $s^{+1}_{l^{+1} -1} = s^n_{l-1}$.   
   Thus, we have  $d^{SR}(Node, s^{+1}_{l^{+1} - 1}, s'^{+1}_{l'}) + d^{SR}(Node,s'^{+1}_{l'},v) = d^{SR}(Node, s^{+1}_{l^{+1}}, v)$, meaning that condition (i) is verified.\\

   \textbf{Consequently, a strongly dominated distance d' remains strongly dominated.}

    \end{IEEEproof}
\end{Lemma}



From Lemma~\ref{lem:extdom}, we can deduce the following theorem : 


\begin{Theorem}
    Extending all non-strongly dominated segment list that have been computed through strong encoding allows to retrieve the entirety of the Pareto front of distances, considering cost, delay, and number of segments.
    \begin{IEEEproof}
        As all non-dominated distances are segment lists, each non-dominated $(cost, delay)$ vector are found. We must then ensure that the minimal segment list will be found for each of these vectors. 

        We know that any given segment list encoding these distances strongly encodes a path (including the minimal segment list). Indeed, let $S$ be a segment list. For any segment $S_i$, we know that there necessarily exists a path $p_i$ from $s_i$ to $s_{i+1}$ such that $d(p_i) = d^{SR}(S_i)$, which is either the shortest path with the highest delay from $s_i$ to $s_{i+1}$ if $t_i = Node$, or a given link if $t_i = Adj$. Thus, $S$ strongly encodes $p_0 \oplus p_1 \oplus \dots \oplus p_l$.

        Clearly, strongly encoding all paths of a given $(cost, delay)$ distance would then enable to find the minimal segment list encoding this distance. 

        While we do not strongly encode \emph{all} of such paths (as not all paths are extended), we showed through Lemma~\ref{lem:extdom} that the paths that are not extended (\ie strongly dominated paths) would necessarily have required a higher or equal number of segment to encode. 

        Consequently, we visit enough path to ensure that the minimal segment list encoding any given distance is found, and so that the entire Pareto front is retrieved.

    \end{IEEEproof}
\end{Theorem}








\noindent 
In this section, we presented \lca, an SR conversion scheme that \emph{strongly} encode paths, an encoding paradigm allowing to leverage load-balancing. Furthermore, we exhibited the peculiarities of the segment metric. From the latter, we derived the notion of strong dominance, which allows pruning paths from the exploration while ensuring to capture the entirety of the Pareto front. By relying on \lca and the concept of strong dominance, multi-criterion path computation algorithms can be modified to correctly take into account the number of segments as a new dimension while exploring the original graph. 


Note, however, that while the overhead induced by \lca is limited, the number of additional (dominated) distances to maintain may be quite high, with no guarantee that the latter will indeed end up on the Pareto front. For some algorithms, directly exploring the SR graph may be more efficient.

